SpikeNeRF: Learning Neural Radiance Fields from Continuous Spike Stream

Spike cameras, leveraging spike-based integration sampling and high temporal resolution, offer distinct advantages over standard cameras. However, existing approaches reliant on spike cameras often assume optimal illumination, a condition frequently unmet in real-world scenarios. To address this, we introduce SpikeNeRF, the first work that derives a NeRF-based volumetric scene representation from spike camera data. Our approach leverages NeRF's multi-view consistency to establish robust self-supervision, effectively eliminating erroneous measurements and uncovering coherent structures within exceedingly noisy input amidst diverse real-world illumination scenarios. The framework comprises two core elements: a spike generation model incorporating an integrate-and-fire neuron layer and parameters accounting for non-idealities, such as threshold variation, and a spike rendering loss capable of generalizing across varying illumination conditions. We describe how to effectively optimize neural radiance fields to render photorealistic novel views from the novel continuous spike stream, demonstrating advantages over other vision sensors in certain scenes. Empirical evaluations conducted on both real and novel realistically simulated sequences affirm the efficacy of our methodology. The dataset and source code are released at https://github.com/BIT-Vision/SpikeNeRF.

==> sec/3_background.tex <==
\section{Background}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

\subsection{Neural Radiance Fields}
Inspired by NeRF which is trained to accumulate the volumetric information with 2D supervision. 
The supervision signal for NeRF is the total squared error between the rendered and true pixel colors.
Basically the neural network $F_\theta(\cdot)$ receives the input of the 3D coordinate $x_i$ and the ray direction $d_i$
3
and the
ray direction di ∈ S
2
and outputs the density σi ∈ R and
emitted radiance ci ∈ R
3

The core of NeRF is to learn 3D volume representation via MLP. Its input is 3D position $\mathbf{o}$ and 2D ray direction $\mathbf{d}$, and the output is color $\mathbf{c}$ and density $\sigma$. As shown in Eq.~\eqref{eq:1}, $F_{\mathbf{\theta}}$ is the MLP network and $\mathbf{\theta}$ is parameters of the network:

\begin{equation}
(\mathbf{c},\sigma) = F_{\mathbf{\theta}}(\gamma_{o}(\mathbf{o}),\gamma_{d}(\mathbf{d})).
\label{eq:1}
\end{equation}

The $\gamma_{o}(\cdot)$ and $\gamma_{d}(\cdot)$ functions are defined in Eq.~\eqref{eq:2}, which map the input 5D coordinates into a higher dimension space. The encoder enables the neural network to better learn the color and geometry information in the scene. And we set $M=10$ for position $\mathbf{o}$, $M=4$ for direction $\mathbf{d}$:

\begin{equation}
\gamma_{M}(x) = \{\sin(2^{m}\pi{x}), \cos(2^{m}\pi{x})\}_{m=0}^{M}.
\label{eq:2}
\end{equation}

To get views from the scene representation, NeRF uses classical volume rendering method as shown in Eq.~\eqref{eq:3}. For a given ray $\mathbf{r}(t)=\mathbf{o}+l\mathbf{d}$ emitting from camera, its expected color projected on the pixel is $C(\mathbf{r})$. $l_{n}$, $l_{f}$ are the near and far bounds of the ray. NeRF divides $[l_{n}, l_{f}]$ into $N$ discrete bins and $\mathbf{c}_{i}$, $\sigma_{i}$ are the output of  $F_{\mathbf{\theta}}$, indicating the color and density of each bin through which the ray passes. $\delta_{i}=l_{i+1}-l_{i}$ is the distance between adjacent samples. $T_{i}$ is the transparency of the particles between $l_{n}$ and bin $i$.

\begin{equation}
    \begin{aligned}
        C(\mathbf{r}) = \sum_{i=1}^{N}T_{i}(1-\exp(-{\sigma}_i{\delta}_i))\mathbf{c}_i,\\
        \text{where} \quad T(i) = \exp(-\sum_{j=1}^{i-1}\sigma_{j}\delta_{j}).
    \end{aligned}
\label{eq:3}
\end{equation}

\begin{equation}
    \mathcal{L}= \sum_{\mathbf{r}\in\mathcal{R}}[\|C_{c}(\mathbf{r})-C(\mathbf{r})\|_{2}^{2}+\\
    \|C_{f}(\mathbf{r})-C(\mathbf{r})\|_{2}^{2}].
\label{eq:4}
\end{equation}

In order to achieve reasonable sampling for the final model, NeRF uses the Hierarchical volume sampling strategy, which optimizes the coarse model and the fine model at the same time, and uses the density obtained by the coarse model to determine the sampling weight of the fine model. The final loss of NeRF is defined as Eq.~\eqref{eq:4}, which is a mean squared loss between the predicted color and ground truth color for both the coarse model and the fine model.

\subsection{Spike Sampling Mechanism}
In FSM, the intensity of light is converted into voltage by the photoreceptor~\cite{recon}. 
Once the voltage reaches a predefined threshold, a one-bit spike is output and a signal to reset the integrator is dispatched at the same time. 
This process is quite similar to the integrate-and-fire neuron.
Different luminance stimuli $I$ lead to different spike firing rates, the output and the reset are triggered asynchronously among various pixels.
Typically, the brighter the light, the faster the firing speed:
\begin{equation}
\int Idt \geq \phi.
\label{eq1}
\end{equation}

The raw data from the spike camera is a three-dimensional spike array $D$.
The spike camera only cares about the integration of the luminance intensity and fires spikes in an ultra-high frequency.
At each sampling moment, if a spike is just fired, a digital signal ``1'' (i.e., a spike) is output, otherwise ``0'' is generated.
We define $S_{i,j}(t) \in \{0,1\}$ to represent the spike firing status of pixel $(i,j)$ at the moment $t$.
For simplicity, we use the \textbf{spike plane} to represent the spike signal output by all pixels at a certain moment, while the spike signals generated by a certain pixel is called a \textbf{spike train} (see Fig. \ref{fig6} (a)).

The spike stream can be mapped into an RKHS (reproducing kernel Hilbert space) as continuous-time functions which incorporate a statistical description of spike trains.
Inspired by [] which utilizes RKHS to measure the distance between two event streams, we design a spike-based distance measurement.
The firing times of each spike $\{t_i \in \mathcal{T} | i = 1,2,...,N\}$
